Investigating Robot Dogs for Construction Monitoring: A Comparative Analysis of Specifications and On-site Requirements

Robot dogs are receiving increasing attention in various fields of research. However, the number of studies investigating their potential usability on construction sites is scarce. The construction industry implies several human resource-demanding tasks such as safety monitoring, material transportation, and site inspections. Robot dogs can address some of these challenges by providing automated support and lowering manual effort. In this paper, we investigate the potential usability of currently available robot dogs on construction sites in terms of focusing on their different specifications and on-site requirements to support data acquisition. In addition, we conducted a real-world experiment on a large-scale construction site using a quadruped robot. In conclusion, we consider robot dogs to be a valuable asset for monitoring intricate construction environments in the future, particularly as their limitations are mitigated through technical advancements.

==> background_old.tex <==

%Background:
%\section{Construction Management}
% Fabian
%Construction Management: Fabian 

%\subsection{On-site management}
Construction sites are complex environments that significantly differ from controlled industrial production environments.
Similar to other industries, the objective of construction is that the on-site factors are controlled in such a manner that buildings can be produced in an economically optimal way.
Work, equipment, and resources are decisive in enhancing the on-site production rate \cite{hofstadler2007bauablaufplanung}.
Due to the unique character of construction sites, diverse, robust, and dynamic monitoring approaches are needed \cite{li2016real}.


%\subsection{Construction Monitoring}
% Within the last decade, diverse methods of job-site monitoring have been established and brought to construction sites.
% Even though there have been many studies on monitoring on-site construction environments, there are many unsolved topics, like construction site suitability, robustness, cost, and deployment of such systems  \cite{li2016real}. % Specifically, indoor progress monitoring is a challenging, not solved topic 
% A core part of the studies focuses on safety monitoring and other unique tasks on sites that are not related to progress monitoring \cite{Vaha2013}.
% These studies are often covered as stand-alone projects, neglecting construction surroundings.
% By now, real-world data-driven studies in the context of digital twin construction are missing.


%> Digital Twin Construction
%% MV-Fabian : the next subsection is very general, do we really needed in the paper? maybe we could replace it as a summary paragraph as part of the introduction?
%\subsection{Digital Twin Construction}
%Frameworks like the digital twin construction \cite{sacks2020} support data management once the on-site data is acquired.
%This can assist various management activities, like taking control of resources, materials, and schedule planning \cite{opoku2021digital}.
% put more details 




% MV-Fabian The subsections previous to this one are very general and do not really contribute to answering the research questions. Maybe we should summarize them in the introduction?
%> Previous studies based on robots
%\subsection{Robots and construction}

The amount of research considering the application of robots in construction has grown significantly in recent years \cite{halder2023robots}. %% new Paragraph (MV):
Several companies have emerged that try to adopt a robotic workforce to solve complex, labor-intensive problems. 
Or even more importantly, to relieve humans of doing dangerous work.


%% new Paragraph (MV):
% While most recent studies focus on using  unmanned aerial vehicles (UAVs), unmanned ground vehicles (UGVs) are required to monitor all construction site areas since some places, like indoor areas, can not be covered by UAVs \cite{halder2023robots}. % give more details

Among the different types of unmanned ground vehicles (UGVs) (wheeled, legged, or tracked), only legged robots provide the flexibility necessary to navigate by rugged hills or low-lying wet swamps, which are usually present in construction sites. 
%Compared with traditional inspection robots (wheeled and tracked), quadruped robots have discrete footholds and can adapt to different terrain, such as stairs, steps, slopes, mountains and so on. Equipped with GPS, robotic arm, lidar and other instruments and testing equipment, they can complete a series of work (intelligent construction, survey, search and rescue, security patrol, etc.), and provide patrol inspection, exploration, material transportation and other work and services for petrochemical, electric power, railway and mineral collection.

One of the few studies concentrating on legged-robot-based progress monitoring demonstrates how a robot can support safety management by tracking the location and size of scaffolding \cite{kim2022deep}.
%However, we could not find comprehensive studies of robot dogs monitoring construction site activity and progress.
Until now, suitability, robustness, cost, and deployment on construction sites of such legged robot systems are open topics.

%\subsection{Constributions}
% MV: I think that the next paragraph would be like the end of the introduction -> reading guide
Therefore, an analysis of the currently available quadruped-legged robots is conducted to inspect their practicality for construction monitoring. %and explore the potential use cases for the construction industry. 
Moreover, a case study for automatic data acquisition with a self-developed mapping system is provided in this paper.

% \subsection{Research questions}
% \begin{itemize}
%     \item Which leg robot dogs are currently available and suitable for supporting construction monitoring?
%     \item How can 3D geometric and semantic data be acquired with a robot dog?
%     \item How can we use BIM models to support the autonomous periodic scanning with robot dogs in construction sites?
%     %\item What are the current challenges which need to be overcome to support the digital twin construction?
%     % - Autonomous navigation is not possible in dynamic and changing environments 
%     % - SLAM Drift 
% \end{itemize}


% MV: I think it would be better if we leave the following instead of the "research questions" which are basically the same, just more clear contributions.
% The following are the main contributions of this paper:
% \begin{itemize}
%     \item A detailed comparison of currently available legged robots and analysis of suitable for supporting construction monitoring.
%     \item A compact mapping system that allows the acquisition of 3D data with UGVs.
%     \item Relevant insights about how the system could support the autonomous creation of digital twins in construction (with semantic and geometric understanding), as well as the challenges that still need to be overcome.
%     % - Autonomous navigation is not possible in dynamic and changing environments 
%     % - SLAM Drift 
% \end{itemize}


%> Potential Usecases?

==> discussion_old.tex <==

In general, to bring robot dogs, specifically the Go1 robot to construction sites, the following challenges should be overcome.
For manual operation, the reliability of the Go1 robot dog was demonstrated to be sufficient in general. 
However, when aiming at autonomous navigation, small problems appeared specifically when launching software updates.
Even though full customer support is provided, the issues proved to be time costly, indicating the prototypical state of the robot.
%Particularly , system reliability is necessary.

On the construction site, we encountered many moving objects and a dynamically changing environment.
These complex conditions lead to inaccuracies in the mapping process, which in turn can cause issues for the robot's autonomous localization and navigation.
Furthermore, due to the presence of high stairway steps or significant slopes, some areas were not reachable for the robot at all and required carrying the robot.
Nonetheless, in these cases, the lighter weight of the Go1 compared to other robot dogs proved to be advantageous.

As most of the construction site is outside, the robot dog has to face diverse temperatures, dust, and rain conditions. 
Unfortunately, the Go1 lacks adequate resistance to these conditions, thereby impeding our ability to conduct further experiments in harsh weather conditions.
% Our problems 
% -> Image resolution (for object detection)
% -> battery capacity
% -> storage capacity

The battery capacity of the robot dog showed a noteworthy limitation.
After around only 30 minutes of exhaustive use, the robot dog's battery was almost empty.
As currently the Go1 cannot be charged automatically, this requires manual effort.
Specifically, at a large construction site, like the presented one, comprehensive autonomous scanning can become an issue.

% The limited battery capacity of the robot dog poses a significant challenge for comprehensive scanning in large construction sites. Due to the battery draining after just 30 minutes of exhaustive use, frequent manual recharging becomes necessary, impeding the efficiency of the scanning process.


%Problems (general)
% -> robot dogs' reliability? 
% -> dynamic construction environment with many obstacles -> always changing environment: autonomous navigation?
% -> weather, temperature?
% -> construction access, climbing? 

% requirements
% - map (BIM model)
% - localization on map, is difficult because of changes in the environment and not updated map representation + dynamic objects.
% -> Waypoints: points of interest 
% - path planning -> traversability ( that the robot can move through the environment)
%Is autonomous data acquisition performed by a robot dog feasible on construction sites?
We believe that at the current state of development of robot dogs, semi-autonomous employment of a quadruped robot is feasible when fulfilling the following requirements:
(1) Comprehensive and reliable 3D BIM models or 3D maps must be available to ensure autonomous localization and navigation.
(2) Major changes to the construction site must continuously be updated on the 3D map.
(3) The deployment of the robot dog should be handled level-wise, avoiding as many barriers as possible.
(4) Precise and fast path planning algorithms are required to allow the robot dogs' autonomous navigation.
(5) Battery capacity should be significantly improved by the manufacturers and a method for autonomous charging should be employed.





    % - Autonomous navigation is not possible in dynamic and changing environments 
    % - SLAM Drift 

==> intro_old.tex <==
% problem statement
Research considering improving digitization on construction sites has increased significantly within the last years \cite{opoku2021digital}.
The digital twin construction, a digital representation of the construction environment, introduces a platform for many construction applications \cite{sacks2020}.
An ongoing challenge is to acquire periodic data of the entire construction site for creating a comprehensive digital twin.

Robot dogs are inspired by the structure and motion of quadruped animals \cite{yao2021design} and usually consist of a body with four mechanical legs allowing use on diverse terrains.

A time-exhaustive task of construction managers is keeping their site projects on track since regular manual site inspections are required. 
In this regard, autonomous robot-based construction monitoring provides a promising approach to reducing the effort.  
Most of the research regarding robot application in construction focuses on unmanned aerial vehicles (UAVs) rather than ground-based, legged robots, which might be a better fit for construction sites \cite{halder2023robots}.

The potential usability of robot dogs on construction sites, focusing on their ability to facilitate data acquisition, access hard-to-reach areas of the site, and sustain with limited power supply options, has to be investigated to embrace future research directions.


% research design
%% MV OLD -> new afterwards
% With our contribution, we present the following items:
% (a) An investigation of potential use cases of legged robot dogs in on-site environments, (b) a summary of state-of-the-art robot dogs, and (c) an on-site experiment unveiling the challenges of legged robot dogs on construction sites.

%% MV New
Overall, this paper offers (a) a detailed comparison of legged robots; (b) presents a compact mapping system for unmanned ground vehicles (UGVs); (c) discusses the potential for autonomous digital twin creation in construction, and identifies the challenges that need to be addressed for successful implementation. These contributions support advancing the use of robotics and mapping technologies in construction monitoring and management.

==> tables/ComparisonTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{cllcccccccccccccllc}
\rowcolor[HTML]{70AD47} 
{\color[HTML]{FFFFFF} \textbf{Nr}} & \multicolumn{1}{c}{\cellcolor[HTML]{70AD47}{\color[HTML]{FFFFFF} \textbf{Name}}} & \multicolumn{1}{c}{\cellcolor[HTML]{70AD47}{\color[HTML]{FFFFFF} \textbf{Company}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Release\\ Year\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}BL\\  (m)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}H\\  (m)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}W\\  (kg)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}PL\\  (kg)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}PLC\\  (\%)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}V\\  (m/s)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{NS}} & {\color[HTML]{FFFFFF} \textbf{NWC}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}C \\ (cm)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}S \\ (deg)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}T \\ (h)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{Prot.}} & \multicolumn{1}{c}{\cellcolor[HTML]{70AD47}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}More\\  info\end{tabular}}}} & \multicolumn{1}{c}{\cellcolor[HTML]{70AD47}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Min P\\   (€)\end{tabular}}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Max P\\   (€)\end{tabular}}} \\
\rowcolor[HTML]{E2EFDA} 
1                                  & A1                                                                               & Unitree                                                                             & 2020                                                                                   & 0,50                                                                              & 0,40                                                                             & 12                                                                                & 7                                                                                  & 58,3                                                                                & 3,3                                                                                & 6,6                                & 385,0                               & 12                                                                                & 35                                                                                 & 1 - 2,5                                                                          & None                                  & link                                                                                                                             & 13.500   €                                                                                                                        & -                                                                                     \\
2                                  & Go1                                                                              & Unitree                                                                             & 2021                                                                                   & 0,65                                                                              & 0,40                                                                             & 12                                                                                & \cellcolor[HTML]{FFFFFF}5                                                          & 41,7                                                                                & 3,7                                                                                & 5,7                                & 239,0                               & 12                                                                                & 35                                                                                 & 1 - 2,5                                                                          & None                                  & \cellcolor[HTML]{E2EFDA}link                                                                                                     & 5.566 €                                                                                                                           & \multicolumn{1}{l}{23.111 €}                                                          \\
\rowcolor[HTML]{E2EFDA} 
3                                  & AlienGo                                                                          & Unitree                                                                             & 2019                                                                                   & 0,65                                                                              & 0,60                                                                             & 20                                                                                & 13                                                                                 & 65,0                                                                                & 1,5                                                                                & 2,3                                & 150,0                               & 18                                                                                & 25                                                                                 & 2,5 - 4,5                                                                        & None                                  & link                                                                                                                             & 44.400 €                                                                                                                          & -                                                                                     \\
4                                  & Spot                                                                             & Boston Dyn.                                                                         & 2020                                                                                   & 1,10                                                                              & 0,61                                                                             & 32                                                                                & 14                                                                                 & 43,8                                                                                & 1,6                                                                                & 1,5                                & 63,6                                & 22                                                                                & 30                                                                                 & 1,5                                                                              & IP54                                  & \cellcolor[HTML]{E2EFDA}{\color[HTML]{0563C1} {\ul link}}                                                                        & {\color[HTML]{FF0000} 75.000 €}                                                                                                   & -                                                                                     \\
\rowcolor[HTML]{E2EFDA} 
5                                  & B1                                                                               & Unitree                                                                             & 2021                                                                                   & 1,10                                                                              & 0,67                                                                             & 50                                                                                & 40                                                                                 & 80,0                                                                                & 1,8                                                                                & 1,6                                & 130,9                               & 20                                                                                & 35                                                                                 & 2 - 4                                                                            & IP68                                  & link                                                                                                                             & 70.000   €                                                                                                                        & \multicolumn{1}{l}{\cellcolor[HTML]{E2EFDA}86.866   €}                                \\
6                                  & ANYmal                                                                           & Anybotics                                                                           & 2019                                                                                   & 0,93                                                                              & 0,89                                                                             & 50                                                                                & 23                                                                                 & 46,0                                                                                & 1,3                                                                                & 1,4                                & 64,3                                & 25                                                                                & 30                                                                                 & 2                                                                                & IP67                                  & \cellcolor[HTML]{E2EFDA}{\color[HTML]{0563C1} {\ul link}}                                                                        & \multicolumn{1}{c}{-}                                                                                                             & \multicolumn{1}{l}{150.000 €}                                                        
\end{tabular}
\end{table}
